Effective Baselines for Multiple Object Rearrangement Planning in Partially Observable Mapped Environments

Many real-world tasks, from house-cleaning to cooking, can be formulated as multi-object rearrangement problems -- where an agent needs to get specific objects into appropriate goal states. For such problems, we focus on the setting that assumes a pre-specified goal state, availability of perfect manipulation and object recognition capabilities, and a static map of the environment but unknown initial location of objects to be rearranged. Our goal is to enable home-assistive intelligent agents to efficiently plan for rearrangement under such partial observability. This requires efficient trade-offs between exploration of the environment and planning for rearrangement, which is challenging because of long-horizon nature of the problem. To make progress on this problem, we first analyze the effects of various factors such as number of objects and receptacles, agent carrying capacity, environment layouts etc. on exploration and planning for rearrangement using classical methods. We then investigate both monolithic and modular deep reinforcement learning (DRL) methods for planning in our setting. We find that monolithic DRL methods do not succeed at long-horizon planning needed for multi-object rearrangement. Instead, modular greedy approaches surprisingly perform reasonably well and emerge as competitive baselines for planning with partial observability in multi-object rearrangement problems. We also show that our greedy modular agents are empirically optimal when the objects that need to be rearranged are uniformly distributed in the environment -- thereby contributing baselines with strong performance for future work on multi-object rearrangement planning in partially observable settings.

==> sections/06_ablation.tex <==
% \begin{table}[h]
%     %\setlength{\tabcolsep}{3.4pt} % Default value: 6pt
%     \fontsize{9pt}{10pt} \selectfont
%     \centering
%     \rowcolors{1}{gray!3}{gray!7}
%     \begin{tabular}{c|cc|cc|cc|cc}
%          & \multicolumn{2}{c|}{GREEDY} & \multicolumn{2}{c|}{L-GAIN} & \multicolumn{2}{c|}{LSTM} & \multicolumn{2}{c}{PRI-C}\\
%         \hline
%         $c$ & 1 & 3 & 1 & 3 & 1 & 3 & 1 & 3\\
%         \hline
%         % $n_o = 1$ & \textbf{.68} & \textbf{.68} & \textbf{.68} & \textbf{.68} & \textbf{.68} & \textbf{.68} & \textbf{.68} & \textbf{.68}\\
%         % \hline
%         % $n_o = 3$ & \textbf{.76} & \textbf{.70} & .75 & .69 & \textbf{.76} & \textbf{.70} & \textbf{.76} & \textbf{.70}\\
%         % \hline
%         % $n_o = 5$ & \textbf{.81} & \textbf{.65} & .80 & \textbf{.65} & .80 & \textbf{.65} & .80 & .64 \\
%         % \hline
%         % $n_o = 10$ & \textbf{.87} & \textbf{.68} & .86 & .66 & .86 & .67 & .84 & .65 \\
%         % \hline
%         $ESPL$ & \textbf{.78} & \textbf{.68} & \textbf{.78} & \textbf{.68} & \textbf{.78} & \textbf{.68} & .77 & .67 \\
%         \hline
%         $\mu_{\Delta ESPL}$ &-&-&.00&.00&.00&.00&.01&.01\\
%         \hline
%         $\sigma_{\Delta ESPL}$&-&-&.10&.09&.01&.01&.05&.06\\
%     \end{tabular}
%     \caption{Comparison of heuristic and ablation agents. All agent uses WFBE$_r$ exploration policy.}
%     \label{tab:ablationvsgreedy}
% \end{table}


\begin{table}[ht!]
    %\setlength{\tabcolsep}{3.4pt} % Default value: 6pt
    \fontsize{9pt}{10pt} \selectfont
    \centering
    \rowcolors{1}{gray!3}{gray!7}
    \begin{tabular}{c| c | c || cc}
        \multicolumn{1}{c}{} & & 
        \multicolumn{1}{c||}{$ESPL$} & \multicolumn{2}{c}{$\Delta ESPL$}\\
        \hline
        \multicolumn{1}{c|}{Methods} & $c$ &
        \multicolumn{1}{c||}{} &
        \multicolumn{1}{c|}{$\mu$} & \multicolumn{1}{c}{$\sigma$}\\
        \hline
        & 1  & \textbf{.78} & - & - \\
        \multirow{-2}{*}{WFBE$_\text{r}$} & 3 & \textbf{.68} & - & -\\
        \hline
        & 1  & \textbf{.78} & .00 & .10 \\
        \multirow{-2}{*}{L-GAIN} & 3 & \textbf{.68} & .00 & .09\\
        \hline
        & 1  & \textbf{.78} & .00 & .01 \\
        \multirow{-2}{*}{LSTM} & 3 & \textbf{.68} & .00 & .01\\
        \hline
        & 1  & .77 & .01 & .05 \\
        \multirow{-2}{*}{PRI-C} & 3 & .67 & .01 & .06\\
    \end{tabular}
    \caption{Comparison of heuristic and ablation agents. All agent uses WFBE$_r$ exploration policy.}
    \label{tab:ablationvsgreedy}
\end{table}



\noindent\textbf{Calculating exact ESPL does not provide significant improvement.} For heuristic agent with WFBE$_r$, we experimented with a different gain calculation (L-GAIN) where we only consider the agent's field-of-view at the target locations instead of calculating the exact gain between agent and target location. This calculation is cheaper and Table \ref{tab:ablationvsgreedy} shows that performance is not significantly effected. This suggests that gains along the way except the target location are not significant on average.

\noindent\textbf{Recursive policy does not do better.} It is a common practice to use recurrent networks for partially observable environments. We use a ConvLSTM-like architecture, substitute final MLP layer of ConvMLP with an LSTM layer, to train OB with a reward function that is 0 for all intermediate steps and $e^{w*ESPL}$ at the end of the episode. Table \ref{tab:ablationvsgreedy} shows that LSTM does not improve the performance. It suggest that agent's state contains all the information that we could remember by utilizing recursive networks.

\noindent\textbf{Privileged critic (PRI-C) can not beat uncorrelated object distribution.} It is also common to have two separate networks for actor and critic algorithms. Since critic network is only used during the training, we can feed object locations to critic and expect it to guide training better. Table \ref{tab:ablationvsgreedy} shows that we do not gain performance improvement even with this technique.

% \noindent\textbf{End to End (E2E) reinforcement learning can not complete episodes.} We also train an agent that consists only primitive actions (\emph{fwd, r45, l45, grab/drop}). During the training, we employ a naive curriculum by starting from small scenes containing a single object. We observe that agent can learn significance of object discovery and navigate towards objects in some episodes. Yet it fails to grab object and navigate to receptacle location in all episodes.
